Uniformization, choice functions and well orders in the class of trees

The monadic second-order theory of trees allows quantification over elements and over arbitrary subsets. We classify the class of trees with respect to the question: does a tree T have a definable choice function (by a monadic formula with parameters)? A natural dichotomy arises where the trees that fall in the first class don't have a definable choice function and the trees in the second class have even a definable well ordering of their elements. This has a close connection to the uniformization problem.

==> mssymb.tex <==

\message{Not using the real mssymb file}
\message{Inputting amssym.def and amssym.tex instead}
 {\catcode`\@11 \global\def\setboxz@h{\setbox0\hbox}
	\global\def\wdz@{\wd0 }
 }

\input amssym.def
\input amssym.tex
\def\napprox{\not\approx}

